Sparsely Activated Mixture-of-Experts are Robust Multi-Task Learners

Traditional multi-task learning (MTL) methods use dense networks that use the same set of shared weights across several different tasks. This often creates interference where two or more tasks compete to pull model parameters in different directions. In this work, we study whether sparsely activated Mixture-of-Experts (MoE) improve multi-task learning by specializing some weights for learning shared representations and using the others for learning task-specific information. To this end, we devise task-aware gating functions to route examples from different tasks to specialized experts which share subsets of network weights conditioned on the task. This results in a sparsely activated multi-task model with a large number of parameters, but with the same computational cost as that of a dense model. We demonstrate such sparse networks to improve multi-task learning along three key dimensions: (i) transfer to low-resource tasks from related tasks in the training mixture; (ii) sample-efficient generalization to tasks not seen during training by making use of task-aware routing from seen related tasks; (iii) robustness to the addition of unrelated tasks by avoiding catastrophic forgetting of existing tasks.

==> background.tex <==
%% Background %%
\subsection{Mixture-of-Experts}
\label{ssec:moe_background}

\subsection{Multi-Task Learning}
\label{ssec:mtl_background}

==> bert_tables.tex <==
%% Table 1: Compare Switch MOE vs MT-DNN vs Single-task baselines vs MMOE for BERT-large
\begin{table*}
\centering
\begin{tabular}{c|cccccccc|c|c} 
\hline
Model & \begin{tabular}[c]{@{}c@{}}RTE\\2.5k\end{tabular} & \begin{tabular}[c]{@{}c@{}}MRPC\\3.6k\end{tabular} & \begin{tabular}[c]{@{}c@{}}STS-B\\5.7k\end{tabular} & \begin{tabular}[c]{@{}c@{}}CoLA\\8.5k\end{tabular} & \begin{tabular}[c]{@{}c@{}}SST-2\\67.3k\end{tabular} & \begin{tabular}[c]{@{}c@{}}QNLI\\104k\end{tabular} & \begin{tabular}[c]{@{}c@{}}QQP\\363k\end{tabular} & \begin{tabular}[c]{@{}c@{}}MNLI\\392k\end{tabular} & \begin{tabular}[c]{@{}c@{}}Small Tasks\\(Avg.)\end{tabular} & \begin{tabular}[c]{@{}c@{}}All tasks\\(Avg.)\end{tabular} \\ 
\hline
BERT-Large & 74.6 & 88.2 & 89.9 & 62.7 & 93.3 & \uline{92.7} & \textbf{91.7} & 86.3 & 78.85 & 84.93 \\
MT-DNN & 83.4 & 87.5 & \uline{90.6} & \uline{63.5} & \textbf{94.3} & \textbf{92.9} & 89.2 & \textbf{86.9} & 81.25 & 86.04 \\ 
\hline
MOE-MTL & \textbf{85.7} & \textbf{88.5} & 90.5 & 61.6 & 93.7 & 92.3 & 91.5 & 86.3 & \uline{81.58} & \uline{86.26} \\
\begin{tabular}[c]{@{}c@{}}\textbf{MMOE-MTL }\end{tabular} & \uline{85.4} & \textbf{88.5} & \textbf{90.8} & \textbf{64.1} & \uline{94.2} & 92.3 & \textbf{91.7} & \uline{86.4} & \textbf{82.20} & \textbf{86.68} \\
\hline
\end{tabular}
\caption{Results on GLUE}
\end{table*}

%% Table 2: Model size vs performance improvement comparison %%
\begin{table*}
\centering
\begin{tabular}{c|c|cc|cc} 
\hline
\multirow{2}{*}{} & \multirow{2}{*}{Params } & \multicolumn{2}{c|}{ Small tasks } & \multicolumn{2}{c}{All Tasks} \\ 
\cline{3-6}
 &  & \multicolumn{1}{c|}{Avg.} & \% change & \multicolumn{1}{c|}{Avg.} & \% change \\ 
\hline
Mini-LM & 1.94x & 74.38 & 3.12\% & 81.83 & 1.30\% \\
BERT-base & 2.55x & 79.98 & 4.51\% & 85.08 & 2.08\% \\
BERT-large & 2.81x & 82.20 & 4.25\% & 86.68 & 2.06\% \\
\hline
\end{tabular}
\caption{Impact of encoder size}
\end{table*}

% Improvements upon single-task baseline and MT-DNN on SciTail
%% Table 3: OOD generalization %%
\begin{table}
\centering
\begin{tabular}{c|c|cc} 
\hline
\multicolumn{2}{c|}{} & 10\% & 100\% \\ 
\hline
\multicolumn{2}{c|}{Bert-base} & 90.5 & 94.3 \\
\multicolumn{2}{c|}{MT-DNN} & 91.1 & 95.7 \\
\multicolumn{2}{c|}{MOE} & 91.3 & 95.0 \\ 
\hline
\hline
\multicolumn{2}{c|}{MMOE-MTL} &  &  \\ 
\cline{1-2}
Head & Gate &  &  \\ 
\hline
Random & Random & 91.0 & 95.9 \\
Random & RTE & 91.6 & 96.0 \\
RTE & RTE & 90.1 & 94.3 \\
\hline
\end{tabular}
\caption{OOD Generalization on SciTail}
\end{table}

%% Table 4: comparing different Hetero-natural with Hetero-uniform for BERT-Large
\begin{table}
\centering
\begin{tabular}{c|cc} 
\hline
\begin{tabular}[c]{@{}c@{}}Task\\Sampling\end{tabular} & \begin{tabular}[c]{@{}c@{}}Small tasks\\(avg.)\end{tabular} & \begin{tabular}[c]{@{}c@{}}All Tasks\\(avg.)\end{tabular} \\ 
\hline
Uniform & 80.60 & 85.75 \\
Natural & \textbf{82.20} & \textbf{86.63} \\
\hline
\end{tabular}
\caption{Results for different task sampling}
\end{table}

%% Table 5: Table showing the trend with change in the number of experts %%
\begin{table}
\centering
\begin{tabular}{c|cc} 
\hline
\begin{tabular}[c]{@{}c@{}}Num. of\\experts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Small tasks\\(avg.)\end{tabular} & \begin{tabular}[c]{@{}c@{}}All Tasks\\(avg.)\end{tabular} \\ 
\hline
2 experts & 80.78 & 85.79 \\
4 experts & \textbf{82.20} & \textbf{86.63} \\
6 experts & 80.60 & 85.76 \\
\hline
\end{tabular}
\caption{Results for variation in number of experts}
\end{table}

==> tables/glue_dataset_stats.tex <==
% \begin{table*}
% \centering
% \begin{tabular}{c|c|c|c|c|c|c} 
% \hline
% Dataset & \#Train & \#Dev & \#Labels & Task & Formulation & Metrics \\ 
% \hline\hline
% STS-B & 5.7k & 1.5k & 1 & Similarity & \begin{tabular}[c]{@{}c@{}}Pairwise-text\\Scoring\end{tabular} & Spearman corr \\ 
% \hline
% COLA & 8.5k & 1k & 2 & Acceptability & \begin{tabular}[c]{@{}c@{}}Single-text\\Classification\end{tabular} & Matthews corr \\
% \hline
% SST-2 & 67.3k & 872 & 2 & Sentiment & \begin{tabular}[c]{@{}c@{}}Single-text\\Classification\end{tabular} & Accuracy \\
% \hline
% MRPC & 3.7k & 408 & 2 & Paraphrase & \begin{tabular}[c]{@{}c@{}}Pairwise-text\\Classification\end{tabular} & Accuracy \\
% \hline
% QQP & 364k & 40k & 2 & Paraphrase & \begin{tabular}[c]{@{}c@{}}Pairwise-text\\Classification\end{tabular} & Accuracy \\ 
% \hline
% RTE & 2.5k & 276 & 2 & NLI & \begin{tabular}[c]{@{}c@{}}Pairwise-text\\Classification\end{tabular} & Accuracy \\ 
% \hline
% QNLI & 105k & 5.5k & 2 & NLI & \begin{tabular}[c]{@{}c@{}}Pairwise-text\\Classification\end{tabular} & Accuracy \\ 
% \hline
% MNLI & 393k & 9.8k & 3 & NLI & \begin{tabular}[c]{@{}c@{}}Pairwise-text\\Classification\end{tabular} & Accuracy \\
% \hline
% \end{tabular}
% \caption{Dataset statistics}
% \label{tab:dataset_stats}
% \end{table*}

\begin{table*}
\centering
\begin{tabular}{cccccc}
\toprule
Dataset & \#Train & \#Dev & \#Labels & Formulation & Metrics \\ 
\midrule\midrule
\multicolumn{6}{c}{\textbf{Similarity}} \\ 
\midrule
STS-B & 5.7k & 1.5k & 1 & \begin{tabular}[c]{@{}c@{}}Pairwise-text\\Regression\end{tabular} & Spearman corr \\ 
\midrule\midrule
\multicolumn{6}{c}{\textbf{ Acceptability }} \\ 
\midrule
COLA & 8.5k & 1k & 2 & \begin{tabular}[c]{@{}c@{}}Single-text\\Classification\end{tabular} & Matthews corr \\ 
\midrule\midrule
\multicolumn{6}{c}{\textbf{ Sentiment }} \\ 
\midrule
SST-2 & 67.3k & 872 & 2 & \begin{tabular}[c]{@{}c@{}}Single-text\\Classification\end{tabular} & Accuracy \\ 
\midrule\midrule
\multicolumn{6}{c}{\textbf{ Paraphrase }} \\ 
\midrule
MRPC & 3.7k & 408 & 2 & \begin{tabular}[c]{@{}c@{}}Pairwise-text\\Classification\end{tabular} & Accuracy \\ 
\midrule
QQP & 364k & 40k & 2 & \begin{tabular}[c]{@{}c@{}}Pairwise-text\\Classification\end{tabular} & Accuracy \\ 
\midrule\midrule
\multicolumn{6}{c}{\textbf{ NLI }} \\ 
\midrule
RTE & 2.5k & 276 & 2 & \begin{tabular}[c]{@{}c@{}}Pairwise-text\\Classification\end{tabular} & Accuracy \\ 
\midrule
QNLI & 105k & 5.5k & 2 & \begin{tabular}[c]{@{}c@{}}Pairwise-text\\Classification\end{tabular} & Accuracy \\ 
\midrule
MNLI & 393k & 9.8k & 3 & \begin{tabular}[c]{@{}c@{}}Pairwise-text\\Classification\end{tabular} & Accuracy \\
\bottomrule
\end{tabular}
\caption{GLUE Dataset details}
\label{tab:dataset_stats}
\end{table*}
